How Transitive Are Real-World Group Interactions? -- Measurement and Reproduction

Many real-world interactions (e.g., researcher collaborations and email communication) occur among multiple entities. These group interactions are naturally modeled as hypergraphs. In graphs, transitivity is helpful to understand the connections between node pairs sharing a neighbor, and it has extensive applications in various domains. Hypergraphs, an extension of graphs, are designed to represent group relations. However, to the best of our knowledge, there has been no examination regarding the transitivity of real-world group interactions. In this work, we investigate the transitivity of group interactions in real-world hypergraphs. We first suggest intuitive axioms as necessary characteristics of hypergraph transitivity measures. Then, we propose a principled hypergraph transitivity measure HyperTrans, which satisfies all the proposed axioms, with a fast computation algorithm Fast-HyperTrans. After that, we analyze the transitivity patterns in real-world hypergraphs distinguished from those in random hypergraphs. Lastly, we propose a scalable hypergraph generator THera. It reproduces the observed transitivity patterns by leveraging community structures, which are pervasive in real-world hypergraphs. Our code and datasets are available at https://github.com/kswoo97/hypertrans.

==> 770Baseline.tex <==

In this section, we present formulae of baseline measures \textbf{B1-6}, which are naive-intuitive approaches (\textbf{B1} and \textbf{B2}) or extensions of measures that are proposed in other studies (\textbf{B3}, \textbf{B4}, \textbf{B5}, and \textbf{B6})~\cite{torres2021and, klamt2009hypergraphs, gallagher2013clustering}.

First, \textbf{B1} and \textbf{B2} are two simple and intuitive measures.

\smallsection{B1. Jaccard index} \textbf{B1} computes the Jaccard similarity between (1) the union of all candidate hyperedges in $C$ and (2) the union of the two wings of $w$.
Formally, 
$$
\mathcal{T}(w, C) = \frac{\lvert \left(\bigcup_{e' \in C} e'\right) \cap (L(w) \cup R(w)) \vert }{\lvert \left(\bigcup_{e' \in C} e'\right) \cup (L(w) \cup R(w)) \vert }.
$$

\smallsection{B2. Ratio of covered interactions} \textbf{B2} computes the ratio of pair interactions in $P(w)$ that are covered by (included in) the candidate hyperedges.
Formally, 
$$
% \mathcal{T}(w, C) = \frac{\left\lvert \left(\bigcup_{e'\in C} {e' \choose 2} \right)  \cap P(w) \right\vert }{\lvert P(w)\vert}.
\mathcal{T}(w, C) = \frac{1}{{\lvert P(w)\vert}} \times {\left\lvert \bigcup_{e'\in C} {e' \choose 2}  \cap P(w) \right\vert }.
$$

Baseline methods \textbf{B3-6} are extensions of existing hypergraph transitivity measures~\cite{torres2021and, gallagher2013clustering, klamt2009hypergraphs}.
Since no existing measures were defined at the hyperwedge level, we extend the concept of local measures (i.e., the local clustering coefficient of a node) to the hyperwedge level.

\smallsection{B3. Klamt et al.~\cite{klamt2009hypergraphs}} \textbf{B3} computes the proportion of candidate hyperedges that intersect with both wings out of those that intersect with at least one wing.  
% checks whether the candidate hyperedges that intersect with one wing also intersect with the other wing. 
Formally,
\begin{equation}
\mathcal{T}(w, C) = \frac{\lvert M(L(w); C) \cap M(R(w); C) \vert}{\lvert M(L(w); C) \cup M(R(w); C)\vert},
\end{equation}
where $M(V'; C) = \{e' \in C : e' \cap V' \neq \emptyset\}$.
Note that if $\not\exists e \in C \ s.t. e \cap (L(w) \cup R(w)) \neq \emptyset$ then we let $\mathcal{T}(w,C) = 0$.


\smallsection{B4. Torres et al.~\cite{torres2021and}} \textbf{B4} computes the proportion of {wing-nodes (i.e., nodes that belong to a wing of the target hyperwedge)} that {are} in the same candidate hyperedge with a node in the other wing.
Formally,
\begin{equation}
    \mathcal{T}(w, C) = \frac{\lvert L(w) \cap \mathcal{N}(R(w); C)\vert + \lvert R(w) \cap \mathcal{N}(L(w); C)\vert}
    {\lvert L(w) \vert + \lvert R(w) \vert},    
\end{equation}
where $\mathcal{N}(V', C)=\bigcup_{e'\in M(V'; C)} e'$ with $M(V'; C)$ is defined in \textbf{B3}.
% $ = \{e' \in C : e' \cap V' \neq \emptyset\}$.
% \fanchen{A bit hard to understand, add some intuition if possible.}

\smallsection{B5. Gallagher et al. A~\cite{gallagher2013clustering}} 
\textbf{B5} computes the proportion {of pairs of wing-nodes} that co-exist in a candidate hyperedge that is disjoint with the body group $B(w)$ out of {all pairs of wing-nodes.}
% checks whether each node pair from the union of two wings is a subset of any candidate hyperedges.
% Here, it only uses candidate hyperedge which does not overlap with the body group. 
Formally, 
\[
\mathcal{T}(w, C) = \Pr[\exists e' \in \tilde{C}~\text{s.t.}~v_1, v_2 \in e' : v_1, v_2 \in L(w) \cup R(w)],
\]
where $\Tilde{C} = \{e' \in {C}: e' \cap B(w) = \emptyset\}$.
% $$
% \mathcal{T}(w, C) = \frac{2 \times \sum_{\{v'_{1}, v'_{2}\} \in {L(w) \cup R(w) \choose 2}} \mathbbm{I}^{\lnot}_{C}[v'_{1}, v'_{2} , B(w)]}{\lvert L(w) \cup R(w)\vert \times (\lvert L(w) \cup R(w)\vert - 1)}
% $$
% where $\mathbbm{I}^{\lnot}_{C}[v'_{1}, v'_{2} , B(w)] = 1$ if $\exists e' \in C$ s.t $\{v'_{1}, v'_{2}\} \subseteq e'$ and $e' \cap B(w) = \emptyset$.

\smallsection{B6. Gallagher et al. B~\cite{gallagher2013clustering}} 
% This is identical to the \textbf{B5}, except that it only uses candidate hyperedge which overlaps with the body group.
\textbf{B6} is similar to \textbf{B5}, except that the candidate hyperedges that intersect with the body group $B(w)$ are considered, instead of those disjoint with $B(w)$.
\[
\mathcal{T}(w, C) = \Pr[\exists e' \in \hat{C}~\text{s.t.}~v_1, v_2 \in e' : v_1, v_2 \in L(w) \cup R(w)],
\]
where $\hat{C} = \{e' \in {C}: e' \cap B(w) \neq \emptyset\}$.

==> 771ProofofThmProp.tex <==
\subsection{Detailed descriptions of axioms}\label{subsec:detailedaxioms}

We briefly rewind the proposed measure and axioms.
The proposed measure \measure is defined as:
\begin{equation}\label{eq:hypertrans}
\mathcal{T}(w, C; f) =
\sum\nolimits_{\{v'_{1}, v'_{2}\} \in P(w)} 
\frac{\max_{e \in C} f(w, e) \mathds{1}[v'_{1}, v'_{2} \in e]} 
{\lvert P(w) \vert }.
\end{equation}
We describe axioms, which are also presented in the main paper.
\begin{axiombox}[Minimum hyperwedge transitivity]\label{ax:min_hw_trans}
A hyperwedge transitivity of $w$ is globally minimized if and only if there is no candidate hyperedge in $C$ being an overlapping hyperedge.
Formally, $\mathcal{T}(w, C) = 0$ (see Axiom~\ref{ax:hw_bounded}) $\Leftrightarrow$ $C \cap \Omega(w) = \emptyset$.
\end{axiombox}

%[Changes of hyperwedge transitivity by candidate-hyperedge increments]
\begin{axiombox}\label{ax:incre_changes_cands}
In this axiom, we discuss how hyperwedge transitivity should change in different situations when we \textbf{include more hyperedges} in the candidate set $C$.
\end{axiombox}
\begin{enumerate}[wide, label=\textsc{\textbf{Case \arabic*}}:, labelindent=10pt]
    \item \textit{(General) 
    Whenever more hyperedges are included in the candidate set $C$, $w$'s transitivity remains the same or increases.
    Formally, $C \subseteq C' \subseteq E \Rightarrow \mathcal{T}(w , C) \leq \mathcal{T}(w , C')$.}
    
    \item \textit{(Only non-overlapping) 
    When only non-overlapping hyperedges %(i.e., hyperedges that are not overlapping hyperedges) 
    are further included in $C$, $w$'s transitivity remains the same.
    Formally, $(C \subseteq C' \subseteq E) \wedge \Big((C' \setminus C) \cap \Omega(w) = \emptyset\Big)\Rightarrow \mathcal{T}(w , C) = \mathcal{T}(w , C')$.}
    
    \item {\textit{(More interactions covered in total)
    When some hyperedges are further included in $C$ so that more interactions in $P(w)$ are covered, $w$'s transitivity strictly increases.
    Formally, $(C \subseteq C' \subseteq E) \wedge \left(\exists e' \in C': (\binom{e'}{2} \setminus \bigcup_{e \in C} \binom{e}{2}) \cap P(w) \neq \emptyset\right)
     \Rightarrow \mathcal{T}(w , C) <  \mathcal{T}(w , C')$.}}
\end{enumerate}

%[Changes of hyperwedge transitivity by candidate-hyperedge enlargements with wing-nodes]
\begin{axiombox}\label{ax:incre_changes_replacement}
In this axiom, we discuss how hyperwedge transitivity should change in different situations when some candidate hyperedges in $C$ are \textbf{enlarged with wing-nodes}, i.e., replaced by their supersets where the new nodes are from the two wings.\footnote{Formally, for each hyperwedge $w$, a candidate hyperedge $e$ is \textit{enlarged with wing-nodes} (to $e'$) if and only if $e \subseteq e'$ with $\emptyset \neq (e' \setminus e) \subseteq (L(w) \cup R(w))$.}
\end{axiombox}
\begin{enumerate}[wide, label=\textsc{\textbf{Case \arabic*}}:, labelindent=10pt]
    \item \textit{(General) 
    When each $e \in C$ is either kept the same or enlarged with wing-nodes, $w$'s transitivity remains the same or increases.
    Formally, $\Big(\exists$ bijection $g: C \to C'$ s.t 
    % $\Big(e \subseteq g(e) \wedge  (g(e) \setminus e) \subseteq (L(w) \cup R(w)), \forall e \in C\Big) 
    $\big(e \subseteq g(e) \subseteq (e \cup L(w) \cup R(w)), \forall e \in C\big)\Big)
    \Rightarrow \mathcal{T}(w, C) \leq \mathcal{T}(w, C')$.}
    
    \item \textit{(Each candidate more interaction-covering)
    When each $e \in C$ is enlarged with wing-nodes so that it covers more interactions in $P(w)$,
    % , and at least one candidate hyperedge is enlarged so that it covers more pair interactions in $P(w)$, 
    $w$'s transitivity strictly increases.
    Formally, $\Big(\exists$ bijection $g: C \to C'$ s.t
    % $\Big(e \subsetneq g(e) \wedge (g(e) \setminus e) \subseteq (L(w) \cup R(w)) 
    $\big(e \subsetneq g(e) \subseteq (e \cup L(w) \cup R(w))
    \wedge (\binom{g(e)}{2} \setminus \binom{e}{2} ) \cap P(w) \neq \emptyset, \forall e \in C\big)\Big) 
    \Rightarrow \mathcal{T}(w, C) < \mathcal{T}(w, C')$.}
\end{enumerate}

\begin{remark}
    %Axioms~\ref{ax:incre_changes_cands} and \ref{ax:incre_changes_replacement} are essentially different.
    %Note that several baseline measures satisfy only one of them.
    Axiom~\ref{ax:incre_changes_replacement} assumes a \textbf{bijection}, {ensuring that} the enlarged hyperedges do not become equivalent {to any} other hyperedges.
    % Several baseline measures satisfy certain cases, while some do not.
    %\fanchen{Emphasize that Axiom~3 is essential even though similar-looking to Axiom~2 by, e.g., the fact that some measures in Table~2 satisfies Axiom~2 but not 3.}
    %Combining Axioms~\ref{ax:incre_changes_cands} and \ref{ax:incre_changes_replacement}, we can discuss how hyperwedge transitivity should change in some situations when the candidate set $C$ includes more hyperedges and some hyperedges in $C$ are enlarged.
    %Please see Appendix~\ref{} for the details.
    %Moreover, a more general version of Axiom~\ref{ax:incre_changes_wing_nodes} can be found in Appendix~\ref{}.
    %\fanchen{TODO: add these contents in the appendix. The general version is the current version where the candidate set's size can decrease, which is more relaxed/general but less intuitive.}
\end{remark}

\begin{axiombox}[Maximum hyperwedge transitivity]\label{ax:max_hw_trans}
When hyperwedge transitivity of $w$ is globally maximized, there exists at least one $e \in C$ including all the nodes of two wings $L(w)$ and $R(w)$. 
Formally, $\mathcal{T}(w, C) = 1 \Rightarrow \exists e \in C$ s.t $L(w) \cup R(w) \subseteq e$.
\end{axiombox}

\begin{remark}
    Since axioms focus on \textbf{group interaction}, \textsc{Axiom}~\ref{ax:max_hw_trans} indicates that all elements in $P(w)$ should co-exist in a single hyperedge.
\end{remark}

\begin{axiombox}[Boundedness of hyperwedge transitivity]\label{ax:hw_bounded}
    A hyperwedge transitivity function $\mathcal{T}$ should be bounded.
    WLOG, we assume that the value is bounded within $[0, 1]$, i.e.,
    $\mathcal{T}(w, C) \in [0, 1], \forall w \in W, \forall C \in 2^{E} \setminus \{\emptyset\}$.    
\end{axiombox}

We now propose two hypergraph-level axioms.
\begin{axiombox}[Reducibility to graph transitivity]\label{ax:reduce_pairwise_graph}
When the input hypergraph $G = (V, E)$ is a pairwise graph, i.e., $|e| = 2, \forall e \in E$, the hypergraph transitivity $T(G)$ should be equal to (i.e., is reduced to) the graph transitivity~\cite{newman2001random} of $G$.
\end{axiombox}

\begin{axiombox}[Boundedness of hypergraph transitivity]\label{ax:hg_bounded}
A hypergraph transitivity function $T$ should be bounded.
% By Axiom~\ref{ax:reduce_pairwise_graph}, it should be bounded in $[0, 1]$ as the graph transitivity function. 
WLOG,
$T(G) \in [0, 1]$, for every \text{hypergraph $G$}.
\end{axiombox}

\begin{comment}
\mathcal{T}(w, C) :=
\sum_{\{v'_{1}, v'_{2}\} \in P(w)} \frac{ \max_{e \in C}(f(w, e) \times \mathds{1}[v'_{1}, v'_{2} \in e])}
{\lvert L(w) \vert \times \lvert R(w) \vert }
\end{comment}

\subsection{Proof of Theorem~\ref{thm:axiomviolation}}\label{subsec:proofviolation}

Note that Theorem~\ref{thm:axiomviolation} describes unconformity of all baseline measures \textbf{B1-9} where all baseline measures violate at least one of the proposed axioms. 
Formally, Theorem~\ref{thm:axiomviolation} is stated as

\begin{theorem}[{Unconformity} of baseline measures]\label{thm:axiomviolation} %Unsoundness
Each baseline measure (\textbf{B1-9}) violates at least one among Axioms~\ref{ax:min_hw_trans}-\ref{ax:hg_bounded}.
\end{theorem}

We provide several counterexamples of baseline methods for each axiom. 
Here, we assume that \textbf{B7-9} (variants of \measure) use a score function $f$ that is defined in Eq~(5) in the main paper, which is \textit{good} (\textsc{Proposition} 1).

In \textsc{Lemma}~\ref{lem:begin}-\ref{lem:last} we consider a hyperwedge $w = \{\{1, 2, 3\}, \{3, 4, 5\}\}$ and 15 hyperedges $
e_{1} = \{1,2\}, e_{2} = \{1,3\} ,e_{3} = \{1,4\}, e_{4} = \{1,5\}, e_{5} = \{2,4\}, e_{6} = \{2,5\}, e_{7} = \{1,3,4\}, e_{8} = \{1,2,4\}, e_{9} = \{1,2,5\}, e_{10} = \{1,4,5\}, e_{11} = \{2,4,5\}, e_{12} = \{1,2,3,4\}, e_{13} = \{1,2,3,5\}, e_{14} = \{1,3,4,5\}, e_{15} = \{2,3,4,5\}
$.



\begin{lemma}\label{lem:begin}
B1, B5, and B6 can not meet \textsc{Axiom~\ref{ax:min_hw_trans}}.
\end{lemma}
\begin{proof}
Under the following setting, computed transitivity value of \textbf{B1}, \textbf{B5}, and \textbf{B6} are as follows, which are violations of \textsc{Axiom 1}.
\begin{align*}
    \text{\textbf{B1}}&: \mathcal{T}(w, \{e_{1}\}) = 2/4 \neq 0,\\
    \text{\textbf{B5}}&: \mathcal{T}(w, \{e_{7}\}) = 0/6 = 0, \\
    \text{\textbf{B6}}&: \mathcal{T}(w, \{e_{3}\}) = 0/6 = 0.
\end{align*}
\end{proof}

Note that in $\textsc{Axiom}$ 2 and 3, multiple cases are proposed respectively. 
Here, a violation of any of these two cases indicates the violation of the corresponding axiom. 
If certain result $k$ is evidence of the violation of \textsc{Case 2}, we denote this as 
$k \xrightarrow[]{\mathds{V}} \text{\textsc{Case 2}}$.
Note that $k \xrightarrow[]{\mathds{V}} \text{\textsc{Case 2}}$ used in the proof of \textsc{Lemma 2} indicates that the \textsc{Case 2} of \textsc{Axiom 2} is violated.

\begin{lemma}
B1, B3, B5, B6, B7, and B8 can not meet \textsc{Axiom~\ref{ax:incre_changes_cands}}.
\end{lemma}
\begin{proof}
Under the following setting, computed transitivity value of \textbf{B1}, \textbf{B3}, \textbf{B5}, \textbf{B6}, \textbf{B7}, and \textbf{B8} becomes as follows: 
\begin{align*}
    \text{\textbf{B1}}&: \mathcal{T}(w, \{e_{3}\}) = 2/4 <  \mathcal{T}(w, \{e_{1}, e_{3}\}) = 3/4 \xrightarrow[]{\mathds{V}} \text{\textbf{\textsc{Case 2}}},\\
    \text{\textbf{B3}}&: \mathcal{T}(w, \{e_{3}\}) = 1 > \mathcal{T}(w, \{e_{1}, e_{3}\}) = 1/2 \xrightarrow[]{\mathds{V}}  \text{\textbf{\textsc{Case 1, 2}}},\\
    \text{\textbf{B5}}&: \mathcal{T}(w, \{e_{7}\}) = 1/6 = \mathcal{T}(w, \{e_{4}, e_{7}\}) = 1/6 \xrightarrow[]{\mathds{V}}  \text{\textbf{\textsc{Case 3}}},\\
    \text{\textbf{B6}}&: \mathcal{T}(w, \{e_{4}\}) = 1/6 = \mathcal{T}(w, \{e_{4}, e_{7}\}) = 1/6 \xrightarrow[]{\mathds{V}}  \text{\textbf{\textsc{Case 3}}},\\
    \text{\textbf{B7}}&: \mathcal{T}(w, \{e_{3}\}) = 1/16 > \mathcal{T}(w, \{e_{1}, e_{3}\}) = 1/24 \xrightarrow[]{\mathds{V}}  \text{\textbf{\textsc{Case 1, 2}}},\\
    \text{\textbf{B8}}&: \mathcal{T}(w, \{e_{8}\}) = 1/2 = \mathcal{T}(w, \{e_{4}, e_{8}\}) = 1/2 \xrightarrow[]{\mathds{V}}  \text{\textbf{\textsc{Case 3}}}.
\end{align*}
All these baseline methods violate at least one case of \textsc{Axiom 2}.
\end{proof}

\begin{lemma}
B1, B2, B3, B4, B5, and B6 can not meet \textsc{Axiom~\ref{ax:incre_changes_replacement}}.
\end{lemma}
\begin{proof}
Under the following setting, computed transitivity of \textbf{B1}, \textbf{B2}, \textbf{B3}, \textbf{B4}, \textbf{B5}, and \textbf{B6} becomes
\begin{align*}
    \text{\textbf{B1}}&: \mathcal{T}(w, \{e_{3}, e_{6}\}) = 1 =  \mathcal{T}(w, \{e_{9}, e_{10}\}) = 1 \xrightarrow[]{\mathds{V}} \text{\textbf{\textsc{Case 2}}},\\
    \text{\textbf{B2}}&: \mathcal{T}(w, \{e_{3},\cdots, e_{6}\}) = 1 = \mathcal{T}(w, \{e_{8},\cdots, e_{11}\}) = 1 \xrightarrow[]{\mathds{V}}  \text{\textbf{\textsc{Case 2}}},\\
    \text{\textbf{B3}}&: \mathcal{T}(w, \{e_{3}\}) = 1 = \mathcal{T}(w, \{e_{8}\}) = 1 \xrightarrow[]{\mathds{V}}  \text{\textbf{\textsc{Case 2}}},\\
    \text{\textbf{B4}}&: \mathcal{T}(w, \{e_{3}, e_{6}\}) = 1 = \mathcal{T}(w, \{e_{9}, e_{10}\}) = 1 \xrightarrow[]{\mathds{V}}  \text{\textbf{\textsc{Case 2}}},\\
    \text{\textbf{B5}}&: \mathcal{T}(w, \{e_{2}\}) = 0 = \mathcal{T}(w, \{e_{7}\}) = 0  \xrightarrow[]{\mathds{V}}  \text{\textbf{\textsc{Case 2}}},\\
    \text{\textbf{B6}}&: \mathcal{T}(w, \{e_{3}\}) = 0 = \mathcal{T}(w, \{e_{8}\}) = 0 \xrightarrow[]{\mathds{V}}  \text{\textbf{\textsc{Case 2}}}.
\end{align*}
All these baseline methods violate at least one case of \textsc{Axiom 2}.
\end{proof}

Now we show that transitivity values of some baseline measures are maximized even when hyperedges that contain both left and right wings (i.e., $L(w) \cup R(w) \subseteq e$) do not exist in a candidate set. 

\begin{lemma}
B1, B2, B3, B4, B5, and B6 can not meet \textsc{Axiom~\ref{ax:max_hw_trans}}.
\end{lemma}
\begin{proof}
Under the following setting, computed transitivity of \textbf{B1}, \textbf{B2}, \textbf{B3}, \textbf{B4}, \textbf{B5}, and \textbf{B6} becomes as follows, which are violations of \textsc{Axiom 4}.
\begin{align*}
    \text{\textbf{B1}}&: \mathcal{T}(w, \{e_{3}, e_{6}\}) = 1 \\
    \text{\textbf{B2}}&: \mathcal{T}(w, \{e_{3},\cdots e_{6}\}) = 1 \\
    \text{\textbf{B3}}&: \mathcal{T}(w, \{e_{2}\}) = 1 \\
    \text{\textbf{B4}}&: \mathcal{T}(w, \{e_{3}, e_{6}\}) = 1 \\
    \text{\textbf{B5}}&: \mathcal{T}(w, \{e_{8}, \cdots, e_{11}\}) = 1 \\
    \text{\textbf{B6}}&: \mathcal{T}(w, \{e_{12}, \cdots, e_{15}\}) = 1.
\end{align*}
\end{proof}

\begin{lemma}
B9 can not meets \textsc{Axiom~\ref{ax:hw_bounded}}.
\end{lemma}
\begin{proof}
    Let $w = \{\{1,2,3\}. \{3,4,5\}\}$ and $e = \{1, 2, 4, 5\}$.
    Since $f(w,e) = 1$ holds, resulting transitivity value becomes $\mathcal{T}(w,\{e\}) = 1 + 1 + 1 + 1 = 4$.
    The value lies outside $[0, 1]$, which is a violation of the condition of \textsc{Axiom~\ref{ax:hw_bounded}}.
    Thus, \textbf{B9} violates \textsc{Axiom~\ref{ax:hw_bounded}}.
\end{proof}

\begin{lemma}
B6 can not meets \textsc{Axiom~\ref{ax:reduce_pairwise_graph}}.
\end{lemma}
\begin{proof}
In this axiom, we assume a specific pair graph $G$ where
$G = (V = \{1,2,3\}, E = \{\{1, 2\}, \{1, 3\}, \{2, 3\}\})$.
In this clique graph, $T(G) = 1$ should hold.
By definition, candidate hyperedges with a size greater than 2 can make transitivity value of \textbf{B6} non-zero.
However, since none of $e \in E$ include 3 nodes, $T(G)$ becomes zero with \textbf{B6}.
\end{proof}

\begin{lemma}\label{lem:last}
B9 can not meets \textsc{Axiom~\ref{ax:hg_bounded}}.
\end{lemma}
\begin{proof}
In this axiom, we assume a specific hypergraph $G$ where
$G = (V = \{1,2,3,4,5\}, E = \{\{1,2,3\}, \{3,4,5\}, \{1,2,4,5\}\})$.
Here, $T(G)$ with \textbf{B9} becomes $T(G) = (4 + 2 + 2)/3 = 2.667$.
The value lies outside $[0, 1]$, which is a violation of the condition of \textsc{Axiom~\ref{ax:hw_bounded}}.
Thus, \textsc{Axiom~\ref{ax:hg_bounded}} is violated.
\end{proof}

\subsection{Proof of Theorem~\ref{thm:measureaxiom}}~\label{subsec:proofmeasureaxiom}

Note that Theorem~\ref{thm:measureaxiom} states the soundness of \measure by showing that \measure satisfies all the axiom.

\begin{theorem}[Soundness of \measure]\label{thm:measureaxiom}
\measure (Eq~(2)) with a good group interaction score function $f$ 
satisfies \textsc{Axiom 1-7}.
\end{theorem}

We decompose the proof of Theorem~\ref{thm:measureaxiom} by \textsc{Lemma}~\ref{lem:axbegin}-\ref{lem:axlast}.
Note that \textit{good} function $f$ should have the following properties.

\begin{definition}
    A group interaction function $f$ is \textit{\textbf{good}}, if $f$ satisfies the following six properties for each $w$ and $e$:
    \begin{enumerate}[wide, labelindent=5pt]
        \item $f : (w, e) \in [0, 1], \forall w \in W(G), e \in E$.\label{prop:bound}
        \item $e \in \Omega(w) \Rightarrow f(w,e) > 0$.\label{prop:notzero}
        \item $f(w,e) = 1 \Rightarrow L(w) \cup R(w) \subseteq e$.\label{prop:perfect2edge}
        \item $L(w) \cup R(w) = e \Rightarrow f(w,e) = 1$.\label{prop:edge2perfect}
        % \item $e \subseteq e' \wedge ((e'\setminus e) \subseteq L(w) \cup R(w)) \Rightarrow f(w,e) \leq f(w, e')$.\label{prop:grow1}
        \item $e \subseteq e' \subseteq (e \cup L(w) \cup R(w)) \Rightarrow f(w,e) \leq f(w, e')$.\label{prop:grow1}
        % \item $e \subsetneq e' \wedge ((e'\setminus e) \subseteq L(w) \cup R(w)) \wedge e' \in \Omega(w)
        % \newline \indent \Rightarrow f(w,e) < f(w, e')$.\label{prop:grow2}
        \item $e \subsetneq e' \subseteq (e \cup L(w) \cup R(w)) \wedge e' \in \Omega(w) \Rightarrow f(w,e) < f(w, e')$.\label{prop:grow2}
    \end{enumerate}
\end{definition}

We use the above \textsc{Property}~\ref{prop:bound}-\ref{prop:grow2} for proofs.

\begin{lemma} \measure meets \textsc{Axiom}~\ref{ax:min_hw_trans}.\label{lem:axbegin} \end{lemma}
\begin{proof}
    We first show the following statement: $\mathcal{T}(w,C) = 0 \Rightarrow C \cap \Omega(w) = \emptyset$.
    By definition of \measure and \textsc{Property}~\ref{prop:bound} (bounded condition), $\mathcal{T}(w,C) = 0$ is equivalent to 
    \begin{equation}\label{eq:axiom1proofwhenzero}
        \max_{e \in C}(f(w, e) \times \mathds{1}[v'_{1}, v'_{2} \in e]) = 0, \forall \{v'_{1}, v'_{2}\} \in P(w).
    \end{equation}
    Let's assume $C \cap \Omega(w) \neq \emptyset$. 
    Then, $\exists e \in C $ such that $e \in \Omega(w)$ holds, and the indicator function in Eq~(\ref{eq:axiom1proofwhenzero}) yields a value of $1$ for the corresponding $e$. 
    In addition, according to \textsc{Property}~\ref{prop:notzero}, $f(w,e) > 0$ also holds. 
    This results in $\max_{e \in C}(f(w, e) \times \mathds{1}[v'_{1}, v'_{2} \in e]) \neq 0$, where contradiction occurs with Eq~(\ref{eq:axiom1proofwhenzero}).
    Thus, Eq~(\ref{eq:axiom1proofwhenzero}) induces $C \cap \Omega(w) = \emptyset$, which is our objective.

    Now we show the other way around: $C \cap \Omega(w) = \emptyset \Rightarrow \mathcal{T}(w,C)$. 
    Since $\not \exists e \in C : e \in \Omega(w)$, the output of the indicator function for all hyperedges is zero. 
    Thus, all scores are equal to zero, which is equivalent to our objective, $\mathcal{T}(w, C) = 0$.
\end{proof}

\begin{lemma} \measure meets \textsc{Case 1 of Axiom~\ref{ax:incre_changes_cands}}. \end{lemma}
\begin{proof}
    Note that \measure picks a maximum score $f(w,e)$ from $e\in C$.
    Since $C$ is a subset of $C'$, Eq~(\ref{eq:axiom2alwaysgreaterorequal}) holds.
    \begin{equation}\label{eq:axiom2alwaysgreaterorequal}
    \begin{aligned}
    &\max_{e \in C}(f(w, e) \times \mathds{1}[v'_{1}, v'_{2} \in e]) \\
    \leq &\max_{e \in C'}(f(w, e) \times \mathds{1}[v'_{1}, v'_{2} \in e]), \forall \{v'_{1},v'_{2}\} \in P(w).
    \end{aligned} 
    \end{equation}
    We rewrite the main inequality $\mathcal{T}(w,C) \leq \mathcal{T}(w,C')$ as follows:
    \begin{align*}
    &\sum_{\{v'_{1}, v'_{2}\} \in P(w)} \frac{ \max_{e \in C}(f(w, e) \times \mathds{1}[v'_{1}, v'_{2} \in e])}
{\lvert L(w) \vert \times \lvert R(w) \vert } \\
\leq &\sum_{\{v'_{1}, v'_{2}\} \in P(w)} \frac{ \max_{e \in C'}(f(w, e) \times \mathds{1}[v'_{1}, v'_{2} \in e])}
{\lvert L(w) \vert \times \lvert R(w) \vert },
    \end{align*}
    \begin{equation}\label{eq:axiom2finaleq}
        \begin{aligned}
            \equiv &\sum_{\{v'_{1}, v'_{2}\} \in P(w)} { \max_{e \in C}(f(w, e) \times \mathds{1}[v'_{1}, v'_{2} \in e])} \\
            \leq &\sum_{\{v'_{1}, v'_{2}\} \in P(w)} { \max_{e \in C'}(f(w, e) \times \mathds{1}[v'_{1}, v'_{2} \in e])}.
        \end{aligned}
    \end{equation}
    
    By Eq~(\ref{eq:axiom2alwaysgreaterorequal}), Eq~(\ref{eq:axiom2finaleq}) holds. 
    Thus, $\mathcal{T}(w,C) \leq \mathcal{T}(w,C')$ also holds.
\end{proof}

\begin{lemma} \measure meets \textsc{Case 2 of Axiom~\ref{ax:incre_changes_cands}}. \end{lemma}
\begin{proof}
    Since $\not \exists e' \in (C' \setminus C) : e' \in \Omega(w)$, the indicator function yields 0 for all $e' \in C' \setminus C$, which is the minimum value of $f$ (\textsc{Property}~\ref{prop:bound}).
    Since \measure picks a maximum score among the candidate set, $e'$ can not change any transitivity value. 
    Thus, $\mathcal{T}(w,C) = \mathcal{T}(w,C')$ always holds.
\end{proof}

\begin{lemma} \measure meets \textsc{Case 3 of Axiom~\ref{ax:incre_changes_cands}}. \end{lemma}
\begin{proof}
    Denote $P(w,C)$ a set of total pair interactions by a candidate set $C$ that intersects with $P(w)$ (i.e., $P(w,C) = \left(\bigcup_{e \in C} \binom{e}{2}\right) \cap P(w)$).
    Since $C \subseteq C'$ and there exists $e' \in C'$ such that $(\binom{e'}{2} \setminus (\bigcup_{e \in C}\binom{e}{2})) \cap P(w) \neq \emptyset$, the relation $P(w,C) \subsetneq P(w,C') \subseteq P(w)$ holds. 
    At $\mathcal{T}(w,C)$, Eq~(\ref{eq:axiom2zero}) holds due to the indicator function: 
    \begin{equation}\label{eq:axiom2zero}
    \max_{e \in C}(f(w, e) \times \mathds{1}[v'_{1}, v'_{2} \in e]) = 0, \forall \{v'_{1} ,v'_{2}\} \in (P(w,C') \setminus P(w,C)).
    \end{equation}    
    Note that Eq~\ref{eq:axiom2zero} regards $e \in C$, not $e \in C'$.
    Here, due to Property~\ref{prop:notzero} and the definition of $P(w,C')$, Eq~(\ref{eq:axiom2existmorethanzero}) holds.
    \begin{equation}\label{eq:axiom2existmorethanzero}
        \exists \{v'_{1} ,v'_{2}\} \in P(w) \setminus P(w,C) : \max_{e \in C'}(f(w, e) \times \mathds{1}[v'_{1}, v'_{2} \in e]) > 0.
    \end{equation}
    
    Here, we rewrite $\mathcal{T}(w,C)$ as follows:
    \begin{align}
    \sum_{\{v'_{1}, v'_{2}\} \in (P(w,C))} &\frac{ \max_{e \in C}(f(w, e) \times \mathds{1}[v'_{1}, v'_{2} \in e])} {\lvert L(w) \vert \times \lvert R(w) \vert }\label{eq:axiom2case3final1} \\
    +\sum_{\{v'_{1}, v'_{2}\} \in (P(w) \setminus P(w,C))} &\frac{ \max_{e \in C}(f(w, e) \times \mathds{1}[v'_{1}, v'_{2} \in e])} {\lvert L(w) \vert \times \lvert R(w) \vert}.\label{eq:axiom2case3final2}
    \end{align}
    
    In the same way, we rewrite $\mathcal{T}(w,C')$ as follows:
    \begin{align}
    \sum_{\{v'_{1}, v'_{2}\} \in P(w,C)} &\frac{ \max_{e \in C'}(f(w, e) \times \mathds{1}[v'_{1}, v'_{2} \in e])} {\lvert L(w) \vert \times \lvert R(w) \vert }\label{eq:axiom2case3final3} \\
    +\sum_{\{v'_{1}, v'_{2}\} \in (P(w) \setminus P(w,C))} &\frac{ \max_{e \in C'}(f(w, e) \times \mathds{1}[v'_{1}, v'_{2} \in e])} {\lvert L(w) \vert \times \lvert R(w) \vert}.\label{eq:axiom2case3final4}
    \end{align}
    Since $C \subseteq C'$, Eq~(\ref{eq:axiom2case3final1}) $\leq $ Eq~(\ref{eq:axiom2case3final2}) holds because of Eq~(\ref{eq:axiom2alwaysgreaterorequal}). 
    In addition, according to Eq~(\ref{eq:axiom2zero}) and Eq~(\ref{eq:axiom2existmorethanzero}), Eq~(\ref{eq:axiom2case3final1}) $ < $ Eq~(\ref{eq:axiom2case3final2}) holds. 
    Putting these two together, $\mathcal{T}(w,C) < \mathcal{T}(w,C')$ holds.
\end{proof}

\begin{lemma} \measure meets \textsc{Case 1 of Axiom~\ref{ax:incre_changes_replacement}}. \end{lemma}
\begin{proof}
    Let $e^{M}_{\{v'_{1}, v'_{2}\}} $ denotes $ \argmax_{e \in C}(f(w, e) \times \mathds{1}[v'_{1}, v'_{2} \in e])$. 
    Then, according to the setting of an axiom, Eq~(\ref{eq:axiom3induced}) holds. 
    \begin{equation}\label{eq:axiom3induced}
    \exists e'\in C':(e^{M}_{\{v'_{1}, v'_{2}\}} \subseteq e')\wedge((e' \setminus e^{M}_{\{v'_{1}, v'_{2}\}}) \subseteq (L(w) \cup R(w))).
    \end{equation} 
    Denote $e'_{\{v'_{1}, v'_{2}\}} \in C'$ that satisfies the condition expressed in Eq~(\ref{eq:axiom3induced}). 
    Then, Eq~(\ref{eq:axiom3finalcondition}) holds due to \textsc{Property}~\ref{prop:grow1}.
    \begin{equation}~\label{eq:axiom3finalcondition}
  f(w,e^{M}_{\{v'_{1}, v'_{2}\}}) \leq  f(w,e'_{\{v'_{1}, v'_{2}\}}).
    \end{equation}
    By definition, $f(w,e^{M}_{\{v'_{1}, v'_{2}\}}) = \max_{e \in C}(f(w, e) \times \mathds{1}[v'_{1}, v'_{2} \in e])$ holds. 
    By using this equality and Eq~(\ref{eq:axiom3finalcondition}), we derive Eq~(\ref{eq:axiom3case1final1}).
    \begin{equation}\label{eq:axiom3case1final1}
        \max_{e \in C}(f(w, e) \times \mathds{1}[v'_{1}, v'_{2} \in e]) \leq \max_{e' \in C'}(f(w, e') \times \mathds{1}[v'_{1}, v'_{2} \in e']).
    \end{equation}
    Since the result of Eq~(\ref{eq:axiom3case1final1}) holds for an arbitrary $\{v'_{1}, v'_{2}\} \in P(w)$, this can be extended to $\forall \{v'_{1}, v'_{2}\} \in P(w)$. 
    Thus, $\mathcal{T}(w,C) \leq \mathcal{T}(w,C')$ is induced from Eq~(\ref{eq:axiom3case1final1}).
\end{proof}

\begin{lemma} \measure meets \textsc{Case 2 of Axiom~\ref{ax:incre_changes_replacement}}. \end{lemma}
\begin{proof}
    Let $e^{M}_{\{v'_{1}, v'_{2}\}} $ denotes $ \argmax_{e \in C}(f(w, e) \times \mathds{1}[v'_{1}, v'_{2} \in e])$. 
    Then, according to the setting of axiom, Eq~(\ref{eq:axiom3induced2}) holds.
    \begin{equation}\label{eq:axiom3induced2}
    \exists e'\in C':(e^{M}_{\{v'_{1}, v'_{2}\}} \subset e')\wedge((e' \setminus e^{M}_{\{v'_{1}, v'_{2}\}}) \subseteq (L(w) \cup R(w))).
    \end{equation} 
    Denote $e'_{\{v'_{1}, v'_{2}\}} \in C'$ that satisfies the condition expressed in Eq~(\ref{eq:axiom3induced2}). 
    Since $e' \in \Omega(w)$,  we induce Eq~\eqref{eq:axiom3finalcondition2} due to \textsc{Property}~\ref{prop:grow2}.
    \begin{equation}~\label{eq:axiom3finalcondition2}
  f(w,e^{M}_{\{v'_{1}, v'_{2}\}}) < f(w,e'_{\{v'_{1}, v'_{2}\}}).
    \end{equation}
    By definition, $f(w,e^{M}_{\{v'_{1}, v'_{2}\}}) = \max_{e \in C}(f(w, e) \times \mathds{1}[v'_{1}, v'_{2} \in e])$ holds.
    By using this equality and Eq~(\ref{eq:axiom3finalcondition2}), Eq~(\ref{eq:axiom3case1final2}) holds.
    \begin{equation}\label{eq:axiom3case1final2}
        \max_{e \in C}(f(w, e) \times \mathds{1}[v'_{1}, v'_{2} \in e]) < \max_{e' \in C'}(f(w, e') \times \mathds{1}[v'_{1}, v'_{2} \in e']).
    \end{equation}
    Since the result of Eq~(\ref{eq:axiom3case1final2}) holds for an arbitrary $\{v'_{1}, v'_{2}\} \in P(w)$, this can be extended to $\forall \{v'_{1}, v'_{2}\} \in P(w)$. 
    Thus, $\mathcal{T}(w,C) < \mathcal{T}(w,C')$ is induced from Eq~(\ref{eq:axiom3case1final2}).
\end{proof}

\begin{lemma} \measure meets \textsc{Axiom~\ref{ax:max_hw_trans}}. \end{lemma}
\begin{proof}
    By definition of \measure and \textsc{Property}~\ref{prop:bound}, $\mathcal{T}(w,C) = 1$ is equivalent to Eq~(\ref{eq:axiom4equivtoone}).
    % and (\ref{eq:axiom4equivtomax}).
    \begin{align}
        &\max_{e \in C'}(f(w, e) \times \mathds{1}[v'_{1}, v'_{2} \in e]) = 1, \forall \{v'_{1}, v'_{2}\} \in P(w).\label{eq:axiom4equivtoone}
        %\equiv &\exists e \in C : f(w, e) \times \mathds{1}[v'_{1}, v'_{2} \in e] = 1, \forall \{v'_{1}, v'_{2}\} \in P(w)\label{eq:axiom4equivtomax}
    \end{align}
    This indicates there exists $e \in C$ that satisfies $f(w, e) \times \mathds{1}[v'_{1}, v'_{2} \in e] = 1$.
    To this end, $f(w, e) = 1$ and $\mathds{1}[v'_{1}, v'_{2} \in e] = 1$ should hold. 
    By \textsc{Property}~\ref{prop:perfect2edge}, $e \in C$ such that $f(w,e) = 1$ should satisfy $L(w) \cup R(w) \subseteq e$. 
    %Two nodes $v'_{1}, v'_{2}$ belong to the corresponding $e$ since it covers both wings. 
    Thus, Eq~(\ref{eq:axiom4equivtoone}) induces $\exists e \in C : L(w) \cup R(w) \subseteq e$, which is a condition of the axiom.
\end{proof}

\begin{lemma} \measure meets \textsc{Axiom~\ref{ax:hw_bounded}}. \label{lem:hw_bounded}\end{lemma}
\begin{proof} Here, the proof is straightforward as follows.
    \begin{align}
    0& \leq f(w,e) \leq 1, \forall e \in E, \quad \because \text{\textsc{Property~\ref{prop:bound}}}.
    \nonumber\\
    \equiv 0& \leq \max_{e \in C} f(w,e) \leq 1, C \subseteq E. \nonumber\\
    \equiv 0& \leq \max_{e \in C} f(w,e) \times \mathds{1}[v'_{1}, v'_{2}] \leq 1, C \subseteq E, v'_{1},v'_{2} \in V. \nonumber\\
    \equiv 0& \leq \sum_{\{v'_{1},v'_{2}\} \in P(w)}\max_{e \in C} f(w,e) \times \mathds{1}[v'_{1}, v'_{2} \in e ] \leq \lvert P(w) \vert \nonumber\\
    \equiv 0& \leq \sum_{\{v'_{1},v'_{2}\} \in P(w)}\frac{\max_{e \in C} f(w,e)  \times \mathds{1}[v'_{1}, v'_{2} \in e ] }{\lvert L(w)\vert \times \lvert R(w)\vert}  \leq 1. \label{eq:axiom5final}\\
    &\because \lvert L(w)\vert \times \lvert R(w)\vert = \lvert P(w)\vert \nonumber
    \end{align}
    Note that the Eq~(\ref{eq:axiom5final}) is identical to the form of \measure.
\end{proof}

\begin{lemma} \measure meets \textsc{Axiom~\ref{ax:hg_bounded}}. \end{lemma}
\begin{proof}
    Since $\lvert e_{i} \lvert = 2, \forall i = \{1, \cdots ,\lvert E \vert\}$, the size of all wings of $G$ are 1 (i.e., $\lvert L(w)\vert = \lvert R(w)\vert = 1, \forall w \in W(G)$).
    Let $L(w) = \{v'_{1}\}$ and $R(w) = \{v'_{2}\}$. We rewrite $\mathcal{T}(w,C)$ as
    \begin{equation}\label{eq:equaltograph}
    \mathcal{T}(w,C) = \max_{e \in C} f(w,e)  \times \mathds{1}[v'_{1}, v'_{2} \in e].
    \end{equation}
    Here, we rewrite $\mathds{1}[v'_{1}, v'_{2} \in e]$ as follows:
    \begin{equation}\label{eq:axiom6comp1}
        \mathds{1}[v'_{1}, v'_{2} \in e] \equiv \mathds{1}[\{v'_{1}, v'_{2}\} = e] \quad \because \lvert e \vert = 2. 
    \end{equation}
    By Eq~(\ref{eq:axiom6comp1}) and \textsc{Property}~\ref{prop:edge2perfect}, we  rewrite Eq~(\ref{eq:equaltograph}) as follows:
    \begin{equation}\label{eq:finalgraph}
    \mathcal{T}(w) = 
    \begin{cases} 1 & \text{if $\exists e \in E : e = \{v'_{1}, v'_{2}\} $} \\
     0 & \text{else}
    \end{cases}
    \end{equation}
    Eq~(\ref{eq:finalgraph}) indicates that for a hyperwedge $w = \{e_{i}, e_{j}\}, e_{i} = \{v'_{1}, v'_{3}\} \in E$ and $e_{j} = \{v'_{2}, v'_{3}\} \in E$, $\mathcal{T}(w) = 1$ holds if there exists an edge $e_{k} = \{v'_{1}, v'_{2}\} \in E$. 
    In such a case, $e_{i}, e_{j}, e_{k} \in E$, and this is identical to the triangle between $v'_{1}, v'_{2}, \text{ and } v'_{3}$.
    Here, for $w' = \{e_{i}, e_{k}\}$ and $w'' = \{e_{j}, e_{k}\}$, $\mathcal{T}(w') = \mathcal{T}(w'') = 1$ also holds. 
    In sum, for a triangle formed by $e_{i}, e_{j},$ and $e_{k}$, $\mathcal{T}(w) + \mathcal{T}(w') + \mathcal{T}(w'') = 3$ holds.
    Thus, a hypergraph-level measure of \measure is identical to the number of triangles in a hypergraph multiplied by the 3 and divided by the number of hyperwedges, which is identical to that of graph transitivity measure~\cite{wasserman1994social}.
\end{proof}

\begin{lemma} \measure meets \textsc{Axiom 7}.\label{lem:axlast}\end{lemma}
\begin{proof}
    According to \textsc{Lemma}~\ref{lem:hw_bounded}, $0 \leq \mathcal{T}(w) \leq 1$ holds. 
    Thus, 
    \begin{equation}\label{eq:hg_bound_goal}
        0 \leq \sum_{w \in W} \mathcal{T}(w) \leq \lvert W \vert \equiv 0 \leq \frac{1}{\lvert W \vert} \sum_{w \in W}\mathcal{T}(w) \leq 1.
    \end{equation}
    Note that Eq~\eqref{eq:hg_bound_goal} is the condition of \textsc{Axiom}~\ref{ax:hg_bounded}.
\end{proof}

\subsection{Proof of Proposition~\ref{prop:choice}}\label{subsec:proofofchoice}

Note that Proposition~\ref{prop:choice} states that Eq~\eqref{eq:penalizeall} (Eq (2) in the main paper) is \textit{good} (i.e., has \textsc{Property}~\ref{prop:bound}-\ref{prop:grow2}).

\begin{proposition}~\label{prop:choice}
The function $f$ defined in Eq~\eqref{eq:penalizeall} (Eq (2) in the main paper) is good.
% meets \scprop~\ref{prop:bound}-\ref{prop:grow2}.
\end{proposition}
Note that the Eq~(\ref{eq:penalizeall}) is 
\begin{equation}\label{eq:penalizeall}
    f(w, e) = \frac{\lvert L(w) \cap e)\vert \times \lvert R(w) \cap e \vert}{\lvert L(w) \cup (e \setminus R(w))\vert \times \lvert R(w) \cup (e \setminus L(w)) \vert }.    
\end{equation}
We decompose  $f(w,e)$ of Eq~(\ref{eq:penalizeall}) into two parts: 
\begin{align}
    &\frac{\lvert L(w) \cap e \vert}{\lvert L(w) \cup (e \setminus R(w)) \vert},\label{eq:propfirstcomp} \\
    &\frac{\lvert R(w) \cap e \vert}{\lvert R(w) \cup (e \setminus L(w)) \vert}.\label{eq:propsecondcomp}
\end{align}
To prove that Eq~\eqref{eq:penalizeall} is \textit{good}, we show Eq~\eqref{eq:penalizeall} meets all \textsc{Property}~\ref{prop:bound}-\ref{prop:grow2} by proving \textsc{Lemma}~\ref{lem:beginprop}-\ref{lem:endprop}.
\begin{lemma} Eq~(\ref{eq:penalizeall}) meets \textsc{Property}~\ref{prop:bound}\label{lem:beginprop} \end{lemma}
\begin{proof}
    Note that $L(w) \cap e \subseteq L(w) \cup (e \setminus R(w))$ and $R(w) \cap e \subseteq L(w) \cup (e \setminus R(w))$ hold by definition of $L(w)$ and $R(w)$. 
    In addition, the denominator of Eq~(\ref{eq:propfirstcomp}) and (\ref{eq:propsecondcomp}) are non-empty. 
    Thus, $0 \leq$ Eq~(\ref{eq:propfirstcomp}) $ \leq 1$ and $0 \leq$ Eq~(\ref{eq:propsecondcomp}) $ \leq 1$ hold.
    Since Eq~(\ref{eq:penalizeall}) is a product of Eq~(\ref{eq:propfirstcomp}) and (\ref{eq:propsecondcomp}), $0 \leq$ Eq~(\ref{eq:penalizeall}) $\leq 1$ also holds, which is our objective.
    %Here, when $e \not \in \Omega(w)$, Eq~(\ref{eq:penalizeall}) becomes 0. 
    %When $L(w) \cup R(w) = e$, Eq~(\ref{eq:penalizeall}) becomes 1.
\end{proof}

\begin{lemma} Eq~(\ref{eq:penalizeall}) meets \textsc{Property}~\ref{prop:notzero} \label{lem:alwaysnnz}\end{lemma}
\begin{proof}
    When $e \in \Omega(w)$, numerator of both Eq~(\ref{eq:propfirstcomp}) and Eq~(\ref{eq:propsecondcomp}) become greater than 0.
    Thus, Eq~(\ref{eq:penalizeall}) $> 0$ holds.
\end{proof}

For the ease of proof of \textsc{Lemma}~\ref{lem:perfecttoone}-\ref{lem:zerotonon}, we provide an additional lemma and its proof.

\begin{lemma}\label{lem:ifandonlyif} For $f =$ Eq~(\ref{eq:penalizeall}), $f(w,e) = 1 \text{ iff } e = L(w) \cup R(w)$. \end{lemma}
\begin{proof}
    We first proof $f(w,e) = 1 \Rightarrow e = L(w) \cup R(w)$. 
    Since the numerator is a subset of the denominator at both Eq~\eqref{eq:propfirstcomp} and Eq~\eqref{eq:propsecondcomp}, $f(w, e) = 1$ hold \textit{iff} the numerator and denominator are identical. 
    Formally, 
    \begin{equation}\label{eq:total1}
        \begin{aligned}
        f(w,e) \Leftrightarrow &(L(w) \cap e = L(w) \cup (e \setminus R(w))) \wedge \\
                           &(R(w) \cap e = R(w) \cup (e \setminus L(w))).
        \end{aligned}
    \end{equation}
    Let's first assume that $e \cap (V \setminus (L(w) \cup R(w))) \neq \emptyset$. 
    Then, Eq~(\ref{eq:total1}) is violated. Thus, Eq~(\ref{eq:total2}) should hold.
    \begin{equation}\label{eq:total2}
        e \cap (V \setminus (L(w) \cup R(w))) = \emptyset \Rightarrow e \subseteq L(w) \cup R(w).
    \end{equation}
    Now let's assume that $e \subsetneq (L(w) \cup R(w))$. 
    Then, $(L(w) \cap e = L(w) \cup (e \setminus R(w)))$ or $(L(w) \cap e = L(w) \cup (e \setminus R(w)))$ might not hold, which is a violation of Eq~(\ref{eq:total1}).
    Thus, $e = L(w) \cup R(w)$ is induced from the aforementioned contradiction. 
    
    Now we show $L(w) \cup R(w) = e \Rightarrow f(w,e) = 1$.
    In such a case, both Eq~(\ref{eq:propfirstcomp}) and Eq~(\ref{eq:propsecondcomp}) become 1, which result in $f(w,e) = 1$. 
    Thus, $L(w) \cup R(w) = e \Rightarrow f(w,e) = 1$ also holds.
    Since bidirectional relation holds, \textit{iff} condition is satisfied.
\end{proof}

\begin{lemma}\label{lem:perfecttoone} Eq~(\ref{eq:penalizeall}) meets \textsc{Property}~\ref{prop:perfect2edge} \end{lemma}
\begin{proof}
    By \textsc{Lemma}~\ref{lem:ifandonlyif}, $f(w,e) = 1 \Rightarrow e = L(w) \cup R(w)$ holds.
    Note that $e = L(w) \cup R(w)$ is a special case of $L(w) \cup R(w) \subseteq e$, and the proof is done.
\end{proof}

\begin{lemma}\label{lem:zerotonon} Eq~(\ref{eq:penalizeall}) meets \textsc{Property}~\ref{prop:edge2perfect} \end{lemma}
\begin{proof}
    By \textsc{Lemma}~\ref{lem:ifandonlyif}, $e = L(w) \cup R(w) \Rightarrow f(w,e) = 1$ holds.
    Note that this is a statement of \textsc{Property}~\ref{prop:edge2perfect} and the proof is done.
\end{proof}

\begin{lemma} Eq~(\ref{eq:penalizeall}) meets \textsc{Property}~\ref{prop:grow1} \end{lemma}
\begin{proof}
    Let a set difference between $e$ and $e'$ as $V'$. Formally,
    \begin{equation}\label{eq:subsetfromwing}
        V' = (e' \setminus e) \subseteq L(w) \cup R(w).
    \end{equation}
    Here, $f(w,e') = f(w,e \cup V')$ is expressed as
    \begin{equation}\label{eq:prop5oppositeform}
    \begin{aligned}
        f(w, (e \cup V')) &= \frac{\lvert L(w) \cap (e \cup V'))\vert}{\lvert L(w) \cup ((e \cup V') \setminus R(w))\vert} \\
        &\times \frac{\lvert R(w) \cap (e \cup V')\vert}{\lvert R(w) \cup ((e \cup V') \setminus L(w)) \vert}.
    \end{aligned}
    \end{equation}
    By definition of $V'$, denominators of $f(w,e)$ and $f(w,e')$ are identical. 
    Thus, $f(w,e) \leq f(w,e')$, which is our main objective, is equivalent to Eq~\eqref{eq:prop5finalform}.
    \begin{equation}\label{eq:prop5finalform}
    \begin{aligned}
        \equiv &\lvert L(w) \cap e\vert \times \lvert R(w) \cap e \vert \\
        \leq &\lvert L(w) \cap (e \cup V') \vert \times \lvert R(w) \cap (e \cup V') \vert.
    \end{aligned}
    \end{equation}
    By definition of $V'$, Eq~(\ref{eq:prop5finalform}) holds.
\end{proof}

\begin{lemma}\label{lem:endprop}
    Eq~(\ref{eq:penalizeall}) meets \textsc{Property}~\ref{prop:grow2}
\end{lemma}
\begin{proof}
    Let a set difference between $e$ and $e'$ as $V'$. Formally,
    \begin{equation}\label{eq:subsetfromwing2}
        V' = (e' \setminus e) \subseteq L(w) \cup R(w), \ V' \neq \emptyset.
    \end{equation}
    Eq~\eqref{eq:prop5finalform} is similar to the main inequality of \textsc{Property}~\ref{prop:grow2}, except for $\leq$, which should be $<$. Formally, 
    \begin{equation}\label{eq:prop6finalform}
    \begin{aligned}
        &\lvert L(w) \cap e\vert \times \lvert R(w) \cap e \vert \\
        < &\lvert L(w) \cap (e \cup V') \vert \times \lvert R(w) \cap (e \cup V') \vert.
    \end{aligned}
    \end{equation}
    By definition of $V'$ and the fact that $e' \in \Omega(w)$ holds, the following inequality (Eq~\eqref{eq:lastineq}) also holds.
    \begin{equation}\label{eq:lastineq}
     \lvert L(w) \cap (e \cup V') \vert \times \lvert R(w) \cap (e \cup V') \vert > 0  \because \text{\textsc{Lemma}~\ref{lem:alwaysnnz}}.
    \end{equation}
    By definition of $V'$ and Eq~\eqref{eq:lastineq},  Eq~\eqref{eq:prop6finalform} is guaranteed.
\end{proof}

\begin{comment}
    \begin{figure*}[t]
       \centering
       \caption{Relations between node degree and node transitivity on the entire real-world hypergraphs (observation~\ref{obs:node}). \label{fig:allnodeobs}}
       \includegraphics[width=0.93\textwidth]{FIG/RealNodeTotal.pdf}
    \end{figure*}
\end{comment}
\subsection{Proof of Theorem~\ref{thm:exactness}}~\label{subsec:proofexact}

Note that Theorem~\ref{thm:exactness} states the exactness of \fastmeasure.
\begin{theorem}[Exactness]\label{thm:exactness}
Given any $w, C, f$, \fastmeasure outputs $\mathcal{T}(w, C; f)$ as defined in Eq~(\ref{eq:hypertrans}).    
\end{theorem}

\begin{proof}
%Note that a score of a specific candidate hyperedge $f(w, e)$ does not depend on specific pair interactions $\{v'_{1}, v'_{2}\} \in P(w)$.
Note that $\max_{e \in C} f(w,e) \mathds{1}[v'_{i},v'_{j} \in e]$, a term that is inside the summation of Eq~\eqref{eq:hypertrans}, is equivalent to $\max_{e\in C_{i,j}} f(w, e)$ where $C_{i,j}$ denotes a set of hyperedges that include both $v_{i}$ and $v_{j}$ since $0 \leq f(w,e) \leq 1$.
%The numerator of Eq~\eqref{eq:hypertrans} is identical to $\max_{e\in C_{i,j}} f(w, e)$ where $C_{1,2}$ is a set consists of candidate hyperedges that include the specific pair interaction $\{v'_{1}, v'_{2}\} \in P(w)$ (i.e., $C_{1,2} = \{e \in C : \{v'_{1}, v'_{2}\} \subseteq e\}$).
%Thus, \measure picks a maximum score among hyperedges that include the specific pair interaction $\{v'_{1}, v'_{2}\}$.
%Denote $P(w, e)$ a subset of $P(w)$ which is included in $e$ (i.e., $P(w,e) = \{\{v'_{1}, v'_{2}\} \in P(w) : \{v'_{1}, v'_{2}\} \subseteq e\}$).
For each $e \in C$, \fastmeasure sequentially compares a score mapped by $\{v'_{i}, v'_{j}\} \in (P(w) \cap \binom{e}{2})$ with the score of the corresponding hyperedge $f(w, e)$. 
The existing value is replaced with $f(w, e)$ if it is smaller than $f(w, e)$. 
%This is identical to the maximum computation procedure via the Brute-Force algorithm.
When the algorithm terminates, a value mapped by a key $\{v'_{i}, v'_{j}\}$ is identical to the $\max_{e\in C_{i,j}} f(w, e)$ since this process is equivalent to the common maximum-searching algorithm.
Thus, computing an average of every mapped value is identical to computing Eq~\eqref{eq:hypertrans} in turn. 
\end{proof}

\begin{algorithm}[t]
\small
\caption{\naivemeasure: a direct computation algorithm for \measure \label{algo:naivemeasure}}
\KwIn{Hyperwedge $w$, candidate set $C$, and score function $f$.}
\KwOut{Hyperwedge transitivity $\mathcal{T}(w, C)$}

$\mathds{T} \leftarrow 0$ \\
\ForEach{$\{v'_{1}, v'_{2}\} \in P(w)$}  { \label{line:forstart2}
    \state $t = 0$ \\
    \ForEach{$e \in C $} {\label{line:algo2pairbegin} 
        \If{$\{v'_{1}, v'_{2}\} \subseteq e$} {
            \state $t = \max(t, \mathcal{T}(w,e))$\label{line:algo2pairend}
        }
    }
    \state $\mathds{T} \leftarrow \mathds{T} + t$
}
\Return $\mathds{T}/\lvert P(w) \vert $
\end{algorithm}


\subsection{Description of \naivemeasure and Proof of Theorem~\ref{thm:fastcomplexity}}\label{subsec:proofcomplexityofmeasure}
We first describe \naivemeasure, which computes \measure as expressed in formula Eq~\eqref{eq:hypertrans}. 
The Pseudocode of \naivemeasure is provided in Algorithm~\ref{algo:naivemeasure}.
For each pairwise elements $\{v'_{1}, v'_{2}\} \in P(w)$ (line~\ref{line:forstart2}), it selects which candidate hyperedge $e \in C$ includes the corresponding $\{v'_{1}, v'_{2}\}$. 
Then, it chooses the maximum $f(w,e)$ among scores of such candidate hyperedges (line~\ref{line:algo2pairbegin}-\ref{line:algo2pairend}).

Now we give a proof of Theorem~\ref{thm:fastcomplexity}.
Note that Theorem~\ref{thm:fastcomplexity} states that the time complexity of \fastmeasure is upper bounded by that of \naivemeasure.

\begin{theorem}[Time complexity]\label{thm:fastcomplexity}
    Given any $w, C, f$, $TC_{fast}(w,C) = \mathcal{O}(TC_{naive}(w,C))$,
    where $TC_{naive}(w,C,f)$ is the time complexity of \naivemeasure,
    and $TC_{fast}(w,C,f)$ is that of \fastmeasure.
    % to compute $\mathcal{T}(w,C)$, and let $TC_{fast}(w,C)$ denote that of \fastmeasure. 
    % Then,  holds.
\end{theorem}

\begin{proof}
    We first compute the complexity of \naivemeasure.
    For a specific $\{v'_{1}, v'_{2}\} \in P(w)$, \naivemeasure should check which candidate hyperedges $e \in C$ is containing $\{v'_{1}, v'_{2}\}$ and picks a maximum score among them.
    This process has a complexity of $\Theta(\lvert C \vert)$.
    The above procedure is performed for every $\{v'_{1}, v'_{2}\} \in P(w)$.
    Consequently, its final complexity with big-$\Theta$ notation becomes 
    \begin{equation}\label{eq:naivealgocomp}
        \Theta(\vert L(w) \vert \times \vert R(w) \vert \times \vert C \vert ) = \Theta\left(\sum_{e \in C} \vert L(w) \vert \times \vert R(w) \vert\right).
    \end{equation}
    
    Now we describe the complexity of \fastmeasure. 
    For a specific $e \in C$, \fastmeasure should first get $\binom{e}{2} \cap P(w)$, which requires $\min(\vert L(w)\vert , \vert e\vert)$ + $\min(\vert R(w)\vert , \vert e\vert)$ complexity. 
    After finding the intersection, \fastmeasure goes through every $\binom{e}{2} \cap P(w)$ and compares the existing value and $f(w,e)$. 
    This requires the complexity of $\vert L(w) \cap e \vert \times \vert R(w) \cap e\vert$.
    In sum, the overall complexity regarding the specific candidate hyperedge $e \in C$ is as follows:
    \begin{equation}\label{eq:totalcomplexityofprop}
        \min(\vert L(w)\vert , \vert e\vert) + \min(\vert R(w)\vert , \vert e\vert) + \vert L(w) \cap e \vert \times \vert R(w) \cap e\vert.
    \end{equation}
    Note that this complexity occurs for each $e \in C$. 
    Now we find the upper bound of Eq~\eqref{eq:totalcomplexityofprop}.
    Since $\lvert L(w) \cap e \vert \leq \min(\vert L(w)\vert , \vert e\vert)$ and $\lvert R(w) \cap e \vert \leq \min(\vert R(w)\vert , \vert e\vert)$ holds, Eq~\eqref{eq:totalcomplexityofprop} $\leq$ Eq~\eqref{eq:boundcomplexityofprop} holds.
    \begin{equation}\label{eq:boundcomplexityofprop}
        \min(\vert L(w)\vert , \vert e\vert) + \min(\vert R(w)\vert , \vert e\vert) + \min(\vert L(w)\vert , \vert e\vert) \times \min(\vert R(w)\vert , \vert e\vert).
    \end{equation}
    By using big-$\mathcal{O}$ notation, we rewrite Eq~\eqref{eq:boundcomplexityofprop} as follows:
    \begin{align}\label{eq:propalgocomp}
        &\mathcal{O}(\min(\vert L(w)\vert , \vert e\vert) + \min(\vert R(w)\vert , \vert e\vert) \nonumber \\
        +&\min(\vert L(w)\vert , \vert e\vert) \times \min(\vert R(w)\vert , \vert e\vert)) \nonumber\\ 
        =&\mathcal{O}(\min(\vert L(w)\vert , \vert e\vert) \times \min(\vert R(w)\vert , \vert e\vert)).
    \end{align}
    Thus, the total complexity of every $e \in C$ becomes as follows:
    \begin{equation}\label{eq:propalgototalcomp}
        \mathcal{O}\left(\sum_{e \in C} \min(\vert L(w)\vert , \vert e\vert) \times \min(\vert R(w)\vert , \vert e\vert)\right).
    \end{equation}
    
    Here, the relationship between terms inside the summation of Eq~\eqref{eq:naivealgocomp} and \eqref{eq:propalgototalcomp} is as follows:
    \begin{equation}\label{eq:compcompare}
        \min(\vert L(w)\vert , \vert e\vert) \times \min(\vert R(w)\vert , \vert e\vert \leq \vert L(w) \vert \times \vert R(w) \vert ,\forall e \in C.
    \end{equation}
    From Eq~\eqref{eq:compcompare} and the fact that Eq~\eqref{eq:naivealgocomp} is about big-$\Theta$ and Eq~\eqref{eq:propalgototalcomp} is about big-$\mathcal{O}$, it is clear that $TC_{full}$ is upper bounded by $TC_{naive}$.
\end{proof}

\begin{comment}
\subsection{Proof of \textsc{Proposition}~\ref{prop:sampling}}~\label{subsec:proofprob}
    \begin{proof}{
    To sample a node $v_{i}$ by \textbf{\texttt{HierarchicalGenerate}}, $L(v)$ should be chosen at the level selection. This probability is equal to $\frac{\alpha^{-L(v_{i})} \lvert \Psi_{L}(L(v))\vert }{\sum_{\ell = 1}^{L'}\alpha^{-\ell} \lvert \Psi_{L}(\ell)\vert}$ where $L' = \max_{v' \in V}L(v')$. 
    Among $\Psi_{L}(L(v))$, a node $v$ should be sampled.
    Since this process is a uniform sampling, the probability of a node being chosen from $\Psi_{L}(L(v))$ is $\frac{1}{\lvert \Psi_{L}(L(v))\vert}$.
    By multiplying two probabilities, we get
    \begin{gather}~\label{eq:probform}
    \frac{\alpha^{-L(v)} \lvert \Psi_{L}(L(v))\vert }{\sum_{\ell = 1}^{L'}\alpha^{-\ell} \lvert \Psi_{L}(\ell)\vert} \times \frac{1}{\lvert \Psi_{L}(L(v))\vert} = \frac{\alpha^{-L(v)}}{\sum_{\ell = 1}^{L'}\alpha^{-\ell} \lvert \Psi_{L}(\ell)\vert}.
    \end{gather}
    Since $\Psi_{L}(\ell)$ is a set of level $\ell$ nodes, it is trivial that $\sum_{\ell = 1}^{L'}\alpha^{-\ell}\lvert \Psi_{L}(\ell)\vert  = \sum_{v' \in V'} \alpha^{-L(v')}$.
    Thus, we can rewrite Eq~(\ref{eq:probform}) by $\frac{\alpha^{-L(v)}}{\sum_{v' \in V'} \alpha^{-L(v')}}$. 
    This is identical to the $\mathcal{P}(v)$. 
    }
\end{proof}
\end{comment}

% \begin{proposition}[Negative correlation between layer index and node degree]
%     \love{For any $v_1, v_2$ with $L(v_1) > L(v_2)$, the expected degree of $v_1$ is smaller than that of $v_2$, i.e., $\mathds{E}(d(v_1)) < \mathds{E}(d(v_2))$.}
% \end{proposition}
% \begin{proof}
%     See Appendix~\ref{subsec:proof_high_level_low_degree}
% \end{proof}
\input{main_alg}


\begin{figure*}[t!]
   \centering
   \caption{Relations between node degree and node transitivity on the entire real-world hypergraphs (observation 3). \label{fig:allnodeobs}}
   \includegraphics[width=0.93\textwidth]{FIG/RealNodeTotal.pdf}
\end{figure*}
\begin{figure*}[t!]
   \centering
   \caption{Relations between node degree and node transitivity on the entire generated hypergraphs by \generator (observation 3).\label{fig:allnodegenobs}}
   \includegraphics[width=0.93\textwidth]{FIG/GenNodeTotal.pdf}
\end{figure*}



\subsection{Proof of \textsc{Proposition}~\ref{prop:high_level_low_degree}}\label{subsec:proof_high_level_low_degree}

Note that Proposition~\ref{prop:high_level_low_degree} indicates that the nodes of lower-level are likely to have higher degrees.
To enhance the reader's understanding, We present a pseudo-code of \generator (Algorithm~\ref{algo:generator}), which is also presented in the main paper.

\begin{proposition}[Negative correlation between layer index and node degree]\label{prop:high_level_low_degree}
    {For any $v_1, v_2$ with $L(v_1) > L(v_2)$ and $\alpha \geq 1$, in a hypergraph generated by \generator (Algorithm~\ref{algo:generator}), the expected degree of $v_1$ is smaller than that of $v_2$, i.e., $\mathds{E}[d(v_1)] < \mathds{E}[d(v_2)]$.}
\end{proposition}

\begin{proof}
    We assume that every layer is fully filled, i.e., each layer $\ell$ consists of exactly $\ell^\beta$ communities, and each contains $C$ nodes.
    Let $T_{max}$ be the maximum layer index.
    This assumption does not affect the statement since only the last layer is possibly incomplete and this can only make the nodes at the last layer, i.e., with the highest level index, have lower expected node degrees.
    For ease of presentation, let $v_{\ell, x, y}$ denote the $y$-th node in the $x$-th community at the $\ell$-th layer.
    For each node $v_{\ell, x, y}$, it is included in a hyperedge in two cases:
    (1) it can be included in an intra-community hyperedge by %\textbf{\texttt{IntraCommunityGenerate}}, or
    \textbf{\texttt{IntraCommunityGenerate}}, or
    (2) it can be included in a hierarchical hyperedge by %\textbf{\texttt{HierarchicalGenerate}}.
    \textbf{\texttt{HierarchicalGenerate}}.
    Note that for all the nodes, the distribution of $AE(\cdot)$ and hyperedge sizes (following $S$) are identical.    
    Formally, let $S_{\ell, x, y}$ be the sequence of the $s$ values for $v_{\ell, x, y}$ as in Line~\ref{line:sample_prep} in Algorithm~\ref{algo:generator}, and the distribution of $S_{\ell, x, y}$ for all the nodes $v_{\ell, x, y}$'s is identical up to permutations.
    For case (1), the expected number of edges for each node $v_{\ell, x, y}$ is the same, which is
    $\mathds{E}_{S_{\ell, x, y}}[1 + (C - 1) q \sum_{s \in S_{\ell, x, y}} \binom{c - 1}{s - 2} / \binom{c - 1}{s - 1}]$.
    Hence, it suffices to check case (2) only.
    For case (2), for each node $v_{\ell, x, y}$,
    the expected number of hyperedges is
    $$\mathds{E}_{S_{\ell, x, y}}[\sum_{\ell' = \ell}^{T_{max}} \sum_{x' = 1}^{\ell'^\beta} \sum_{i' = 1}^{C} \sum_{s \in S_{\ell, x, y}} (1 - q)(1 - (1 - \frac{\alpha^{-\ell}}{\sum_{\ell'' = 1}^{\ell'} \alpha^{\ell} \ell''^{\beta}})^s)],$$
    where the first summation $\sum_{\ell' = \ell}^{T_{max}}$ is strictly decreasing ($\ell'$ has a smaller range) with $\ell$ increasing,
    and all the inner summation is positive and non-increasing with $\ell$ increasing when $\alpha \geq 1$.
    % identical for all the nodes, and the first summation $\sum_{\ell' = \ell}^{T_{max}}$ is strictly decreasing with $l$ increasing, 
\end{proof}


==> 772AllHypergraphProperties.tex <==

\begin{table*}[t!]
\caption{Detailed statistics regarding the reproducibility of various hypergraph properties of our proposed generator \generator and four baseline generative models (HyperPA~\cite{do2020structural}, HyperFF~\cite{ko2022growth}, HyperLap~\cite{lee2021hyperedges}, and HyperLap+~\cite{lee2021hyperedges}). 
We use formulae of each hypergraph property that are explained in Choe et al.~\cite{choe2022midas}.
For statistics that can be summarized as a single scalar, we report the absolute statistics (density and diameter).
For statistics that are represented by a distribution, we report Kolmogorov–Smirnov statistic (D-stat)~\cite{smirnov1948table}, a distributional distance between the distribution of the corresponding statistic of a real-world hypergraph and that of the generated hypergraph (hyperedge size, degree, and intersection size).
Note that the proposed generator \generator's reproducibility of various hypergraph properties is comparable to that of other baseline hypergraph generative models.
}\label{tab:overallpropstat}
    \centering
    \scalebox{0.8}{
    \renewcommand{\arraystretch}{1.0}
        \centering
        \begin{tabular}{c | c| c c c |c c c| c c |c c |c c | c}
            \toprule
            \multirow{2}{*}{\textbf{Statistic}} & \multirow{2}{*}{\textbf{Generator}} & \multicolumn{3}{c|}{coauthorship} & \multicolumn{3}{c|}{q\&a} & 
            \multicolumn{2}{c|}{email} & \multicolumn{2}{c|}{ndc} &  \multicolumn{2}{c|}{contact} & Average \\
            & & dblp & geology & history & ubuntu & math & server & enron & eu & classes & substances & high & primary & ranking \\
            \midrule
            \midrule
            \multirow{7}{*}{\makecell{\textbf{Density} \\ \textbf{(Absolute Value)}}} 
            &\textbf{Real-world} & 1.18 & 0.83 &  0.50 &  1.33 & 2.59 &  1.46 & 10.20 & 24.87 & 0.91 & 1.82 & 23.91 & 52.50 & NA \\

            \cmidrule{2-15}
            &\textbf{\generator} & 1.18 & 1.00 & 1.00 & 1.00 & 2.59 & 1.46 & 10.20 & 24.87 & 1.00 & 1.82 & 23.91 & 52.50 & 1.25 \\
            
            %\midrule
            \cmidrule{2-15}
            &\textbf{HyperPA}~\cite{do2020structural} & - & - & - & 2.47 & - & - & 9.79 & 25.32 & 2.66 & - & 181.81 & 145.81 & 4.50 \\
            
            &\textbf{HyperFF}~\cite{ko2022growth} & 3.24 & 3.23 & 3.24 & 3.23 & 3.23 & 3.23 & 3.49 & 11.09 & 3.62 & 3.20 & 3.02 & 2.95 & 4.08\\
            
            &\textbf{HyperLap}~\cite{lee2021hyperedges} & 1.43 & 1.04 & 0.71 & 1.72 & 2.83 & 1.73 & 10.20 & 24.99 & 0.99 & 1.87 & 23.91 & 52.50 & 1.58\\

            &\textbf{HyperLap+}~\cite{lee2021hyperedges} & 1.47 & 1.09 & 0.72 & 1.89 & 3.42 & 1.98 & 10.20 & 25.54 & 1.08 & 2.15 & 23.91 & 52.50 & 2.50\\
            \midrule 
            \midrule 
            %%%%%%%%%%%%%%%%% Diameter %%%%%%%%%%%%%%%%%
            
            \multirow{7}{*}{\makecell{\textbf{Diameter} \\ \textbf{(Absolute Value)}}} 
            &\textbf{Real-world} & 6.81 & 7.09 & 11.45 & 4.74 & 3.75 & 4.29 & 2.38 & 2.78 & 4.65 & 3.59 & 2.63 & 1.88 & NA \\

            \cmidrule{2-15}
            &\textbf{\generator} & 5.90 & 5.99 & 6.25 & 7.46 & 4.62 & 4.63 & 1.86 & 1.89 & 3.35 & 2.11 & 2.41 & 1.87 &  2.67\\
            
            %\midrule
            \cmidrule{2-15}
            &\textbf{HyperPA}~\cite{do2020structural} & - & - & - & 3.77 & - & - & 1.95 & 1.97 & 2.60 & - & 1.83 & 1.79 & 4.08 \\
            
            &\textbf{HyperFF}~\cite{ko2022growth} & 7.14 & 7.01 & 6.83 & 6.37 & 5.95 & 6.56 & 4.00 & 3.05 & 4.73 & 5.01 & 5.11 & 4.91 & 2.83\\
            
            &\textbf{HyperLap}~\cite{lee2021hyperedges} & 5.32 & 5.08 & 7.17 & 6.48 & 4.23 & 4.83 & 4.00 & 3.05 & 4.73 & 5.01 & 5.11 & 4.91 & 2.58\\

            &\textbf{HyperLap+}~\cite{lee2021hyperedges} & 15.66 & 12.10 & 35.68 & 6.75 & 4.79 & 4.94 & 2.78 & 3.41 & 3.51 & 3.70 & 3.11 & 2.73 & 2.83\\

            \midrule 
            \midrule 

            %%%%%%%%%%%%%%%%% HE Size %%%%%%%%%%%%%%%%%

            \multirow{6}{*}{\makecell{\textbf{Hyperedge Size} \\ \textbf{(D-stat)}}} 
            
            &\textbf{\generator} & 0.003 & 0.002 & 0.001 & 0.306 & 0.037 & 0.003 & 0.123 & 0.257 & 0.024 & 0.011 & 0.249 & 0.281 & 3.67\\
            
            %\midrule
            \cmidrule{2-15}
            &\textbf{HyperPA}~\cite{do2020structural} & - & - & - & 0.301 & - & - & 0.123 & 0.257 & 0.024 & 0.011 & 0.249 & 0.281 & 3.92\\
            
            &\textbf{HyperFF}~\cite{ko2022growth} & 0.381 & 0.397 & 0.063 & 0.306 & 0.056 & 0.104 & 0.143 & 0.186 & 0.470 & 0.561 & 0.106 &  0.186 & 4.17\\
            
            &\textbf{HyperLap}~\cite{lee2021hyperedges} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 1.00\\

            &\textbf{HyperLap+}~\cite{lee2021hyperedges} & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 1.00\\

            \midrule 
            \midrule 

            %%%%%%%%%%%%%%%%% Degree Dist %%%%%%%%%%%%%%%%%

            \multirow{6}{*}{\makecell{\textbf{Degree} \\ \textbf{(D-stat)}}} 
            
            &\textbf{\generator} & 0.500 & 0.555 & 0.564 & 0.489 & 0.709 & 0.499 & 0.378 & 0.569 & 0.691 & 0.667 & 0.373 & 0.347 & 3.91\\
            
            \cmidrule{2-15}
            &\textbf{HyperPA}~\cite{do2020structural} & - & - & - & 0.225 & - & - & 0.343 & 0.322 & 0.064 & - & 0.878 & 0.550 & 3.93\\
            
            &\textbf{HyperFF}~\cite{ko2022growth} & 0.360 & 0.430 & 0.605 & 0.566 & 0.411 & 0.466 & 0.532 & 0.359 & 0.348 & 0.158 & 0.856 &  0.963 & 3.75\\
            
            &\textbf{HyperLap}~\cite{lee2021hyperedges} & 0.244 & 0.266 & 0.326 & 0.308 & 0.251 & 0.264 & 0.119 & 0.043 & 0.244 & 0.141 & 0.024 & 0.029 & 1.25\\

            &\textbf{HyperLap+}~\cite{lee2021hyperedges} & 0.258 & 0.292 & 0.331 & 0.369 & 0.408 & 0.366 & 0.084 & 0.111 & 0.323 & 0.320 & 0.046 & 0.050 & 1.92\\

            \midrule 
            \midrule 

            %%%%%%%%%%%%%%%%% Intersection Size %%%%%%%%%%%%%%%%%

            \multirow{6}{*}{\makecell{\textbf{Intersection Size} \\ \textbf{(D-stat)}}} 
            
            &\textbf{\generator} & 0.675 & 0.643 & 0.412 & 0.200 & 0.508 & 0.250 & 0.231 & 0.195 & 0.167 & 0.414 & 0.417 & 0.250 & 3.00\\
            
            %\midrule
            \cmidrule{2-15}
            &\textbf{HyperPA}~\cite{do2020structural} & - & - & - & 0.300 & - & - & 0.255 & 0.234 & 0.280 & - & 0.250 & 0.250 & 3.83\\
            
            &\textbf{HyperFF}~\cite{ko2022growth} & 0.267 & 0.275 & 0.308 & 0.200 & 0.444 & 0.167 & 0.385 & 0.249 & 0.482 & 0.250 & 0.333 &  0.500 & 3.08\\
            
            &\textbf{HyperLap}~\cite{lee2021hyperedges} & 0.233 & 0.315 & 0.227 & 0.300 & 0.333 & 0.233 & 0.192 & 0.222 & 0.357 & 0.214 & 0.250 & 0.250 & 1.92\\

            &\textbf{HyperLap+}~\cite{lee2021hyperedges} & 0.259 & 0.315 & 0.227 & 0.333 & 0.278 & 0.233 & 0.231 & 0.195 & 0.167 & 0.414 & 0.417 & 0.250 & 2.42\\


            \bottomrule
        \end{tabular}
        }
\end{table*}


\subsection{Additional experimental results regarding Observation 3}
In the main paper, we discuss the relationship between the node degree and node transitivity.
Specifically, the average transitivity of nodes decreases as the node degree increase, while such trends cannot be observed on their random counterpart (refer to {Observation}~3 in the main paper). 
In addition, \generator has successfully reproduced this pattern (refer to Section 5.2 of the main paper). 
In this subsection, we present additional experimental results that demonstrate such patterns in the entire dataset.

As shown in Figure~\ref{fig:allnodegenobs}, Observation 3 in the main paper has been discovered in 10 out of 12 datasets, where such a pattern is not clear in NDC-classes and NDC-substances datasets.
In addition, as shown in Figure~\ref{fig:allnodegenobs}, \generator has successfully reproduced Observation 3 in datasets where such a pattern is clearly observed.

\subsection{Reproduction of other properties}
In this subsection, we present detailed experimental results on how well the proposed generator \generator and other baseline generators including HyperPA~\cite{do2020structural}, HyperFF~\cite{ko2022growth}, HyperLAP~\cite{lee2021hyperedges}, and HyperLAP+~\cite{lee2021hyperedges} reproduce various properties of real-world hypergraphs.
We examine density, diameter, hyperedge size, degree, and intersection size.
For density and diameter, we have reported the value of each statistic in real-world and generated hypergraphs, and the ranks of each generator have been measured according to the absolute difference between the statistic of real-world hypergraphs and that of generated hypergraphs.
For hyperedge size, degree, and intersection size, since they are distribution, we have reported D-statistic between the distribution of the real-world and that of the generated hypergraphs. 
Here, ranks are measured according to how small the corresponding D-statistic is (i.e., how close the distribution of generated hypergraphs' statistics are to that of real-world hypergraphs).
Detailed results are reported in Table~\ref{tab:overallpropstat}.
As explained in Appendix C of the main paper, \generator shows outperforming or competitive results on various hypergraph properties, compared to other (including both incremental and static) hypergraph generators. 
In addition, it outperforms other incremental generators including HyperPA and HyperFF in most properties.

==> 773ComplexGenOthers.tex <==
In this subsection, we provide a detailed complexity analysis of used baseline generators.
Refer to Appendix C.3 and Table 10 of the main paper regarding the complexity.

\smallsection{Complexity of HyperPA~\cite{do2020structural}} {HyperPA} is an incremental generator that has its basis on preferential attachment.
It samples a group of nodes proportional to the group degree and composes a hyperedge with the sampled group.
Here, since there may exist $\binom{\vert V\vert}{\vert e\vert - 1}$ number of possible candidates that can be sampled\footnote{A newly introduced node should be included, and this results in sampling $\vert e\vert - 1$ number of nodes}, the time complexity of HyperPA for generating a size $\vert e\vert$ hyperedge is equivalent to $\mathcal{O}(\log_{2}{\binom{\vert V\vert}{\vert e\vert}})$.\footnote{Note that weighted sampling requires $\mathcal{O}(\log_{2}{n})$.}
In sum, the time complexity of HyperPA in generating a hypergraph with given statistics is equivalent to $\mathcal{O}\left(\sum_{e \in E}\log_{2}{\binom{\vert V\vert }{\lvert e \vert}}\right)$.

Regarding memory, it should save all subsets of each generated hyperedge.
Thus, memory complexity of HyperPA is equivalent to $\mathcal{O}\left(\sum_{e \in E} 2^{\lvert e \vert }\right)$.
Due to its exponential memory complexity, {HyperPA} often fails in replicating large-scale hypergraphs (see Table 7 of the main paper). 

\smallsection{Complexity of HyperFF~\cite{ko2022growth}} \textbf{HyperFF} is an incremental generator that selects an ambassador from the existing nodes and includes neighboring nodes of the ambassador in a stochastic way (spec., according to two hyperparameters $p$ and $q$). 
In the worst case, to make a hyperedge with a size of $\vert e\vert$, it may visit every node as many times as $\vert e\vert$.
Thus, the time complexity of HyperFF for generating a size $\vert e\vert$ hyperedge is equivalent to $\mathcal{O}(\lvert V \vert \times \lvert e \vert)$.
In sum, the time complexity of HyperFF in generating a hypergraph with given statistics is equivalent to $\mathcal{O}\left(\lvert V \vert \times \sum_{e \in E} {\lvert e \vert} \right)$.
%Since its complexity is proportional to the multiplication of the number of nodes and the number of hyperedges, it fails in generating large-scale hypergraphs at certain hyperparameter settings, as pointed out by Lee et al.~\cite{lee2021hyperedges} and our preliminary experiments.

Regarding memory complexity, HyperFF only requires space for generated nodes and hyperedges. 
Thus, the memory complexity of HyperFF is equivalent to $\mathcal{O}(\lvert V \vert + \sum_{e \in E} \lvert e \vert)$.

\smallsection{Complexity of HyperLap and HyperLap+~\cite{lee2021hyperedges}}
Regarding the time and memory complexity of HyperLap and HyperLap+, We follow the complexity analysis provided by Lee et al.~\cite{lee2021hyperedges}.
